On Explaining Multimodal Hateful Meme Detection Models

Hateful meme detection is a new multimodal task that has gained significant traction in academic and industry research communities. Recently, researchers have applied pre-trained visual-linguistic models to perform the multimodal classification task, and some of these solutions have yielded promising results. However, what these visual-linguistic models learn for the hateful meme classification task remains unclear. For instance, it is unclear if these models are able to capture the derogatory or slurs references in multimodality (i.e., image and text) of the hateful memes. To fill this research gap, this paper propose three research questions to improve our understanding of these visual-linguistic models performing the hateful meme classification task. We found that the image modality contributes more to the hateful meme classification task, and the visual-linguistic models are able to perform visual-text slurs grounding to a certain extent. Our error analysis also shows that the visual-linguistic models have acquired biases, which resulted in false-positive predictions.

==> Methodology.tex <==

\begin{figure*}[h]
    \centering
    \includegraphics[width=1\textwidth]{images/slurs-grounding-goats.jpg}
    \caption{Placeholder for framework}
    \label{fig:xmultihate-framework}
\end{figure*}

To address our research questions, we propose a post-hoc explanation framework that uses multiple state-of-the-art model interpretation techniques \textcolor{red}{collectively} - XMultiHate. Our framework provides researchers a systematic approach to analyse the various inputs for visual-linguistic models independently and interactively.

For independent analysis, our framework calculates the contribution of each modality towards making models' decisions via two interpretation approaches - attention-based (explicit) and gradient-based (implicit) approaches. Furthermore, our framework displays the individual text and visual segments that contributes the most towards making the model's decision via the gradient-based approach (i.e. Integrated Gradient and Gradient-Based Ranking respectively). This allows researchers to \textcolor{red}{???}

For interactive analysis, our framework allows researchers to inspect the contribution

\subsection{Integrated Gradient}

\begin{equation}
IntegratedGradients_i(x) ::= (x_i - x_{i}^{'}) \times \int^{1}_{\alpha=0} \frac{\partial F(x^{'} + \alpha \times (x - x^{'})}{\partial x_i} d\alpha
\end{equation}

==> Related.tex <==
\subsection{Hateful Memes Classification}
With the recent surge of interest in multimodal problems, multimodal memes have become the key area for multimodal reasoning and understanding in many downstream tasks \cite{suryawanshi2020multimodal, kiela2020hateful, pramanick2021detecting}. 

\subsection{Neural Network Interpretation Techniques}
Neural network interpretation such as the prominent work (BERT and What does BERT with vision look at)

\textbf{Gradient-Based Approach}. Coming soon... Cite Saliency, GradCAM and Integrated Gradients (Text-Based Analysis)

\textbf{Attention-Based Approach}. Coming soon... Cite BERT 

\subsection{Vision-And-Language Modal And Analysis}
Existing researches have examined the contribution of individual evidences in vision-and-language pretraining tasks by hiding certain signals from a specific modality (i.e. masking certain keywords or region of the images) and observing the fluctation in the model's prediction \cite{frank2021vision, srinivasan2021worst}.

Transition into the importance of Vision-And-Model Analysis. Cite popular works such as "What does BERT with Vision look at" and "Vision-and-Language Or Vision-For-Language"

\textbf{Multi-Modal Models}. Visual BERT and VilBERT

\textbf{Existing Analysis}. What does BERT with Vision look at and Vision-and-Language or Vision-For-Language




